On the Power and Limitations of Branch and Cut

The Stabbing Planes proof system was introduced to model the reasoning carried out in practical mixed integer programming solvers. As a proof system, it is powerful enough to simulate Cutting Planes and to refute the Tseitin formulas -- certain unsatisfiable systems of linear equations mod 2 -- which are canonical hard examples for many algebraic proof systems. In a recent (and surprising) result, Dadush and Tiwari showed that these short refutations of the Tseitin formulas could be translated into quasi-polynomial size and depth Cutting Planes proofs, refuting a long-standing conjecture. This translation raises several interesting questions. First, whether all Stabbing Planes proofs can be efficiently simulated by Cutting Planes. This would allow for the substantial analysis done on the Cutting Planes system to be lifted to practical mixed integer programming solvers. Second, whether the quasi-polynomial depth of these proofs is inherent to Cutting Planes. In this paper we make progress towards answering both of these questions. First, we show that any Stabbing Planes proof with bounded coefficients SP* can be translated into Cutting Planes. As a consequence of the known lower bounds for Cutting Planes, this establishes the first exponential lower bounds on SP*. Using this translation, we extend the result of Dadush and Tiwari to show that Cutting Planes has short refutations of any unsatisfiable system of linear equations over a finite field. Like the Cutting Planes proofs of Dadush and Tiwari, our refutations also incur a quasi-polynomial blow-up in depth, and we conjecture that this is inherent. As a step towards this conjecture, we develop a new geometric technique for proving lower bounds on the depth of Cutting Planes proofs. This allows us to establish the first lower bounds on the depth of Semantic Cutting Planes proofs of the Tseitin formulas.

==> EquivalenceLinSP.tex <==




%That is, a linear $\SP$ proof is a restriction of an $\SP$ proof to require that at least one child of every node in the $\SP$ refutation is the empty polytope. 
\begin{figure}[H]
		\centering
		\begin{tikzpicture}

		\draw[thick, ->] (0,0)  -- (1,-1);
		\draw[thick, ->] (0,0)  -- (-1,-1);
		\filldraw[fill=white,thick] (0,0) circle (3pt);
		\draw[thick, ->] (1.1,-1.1)  -- (0.1,-2.1);
		\draw[thick, ->] (1.1,-1.1)  -- (2.1,-2.1);
		\filldraw[fill=white,thick] (1.1,-1.1) circle (3pt);
		\draw[thick, dotted] (2,-2)  -- (3,-3);
		\draw[thick, ->] (3.1,-3.1)  -- (4.1,-4.1);
		\draw[thick, ->] (3.1,-3.1)  -- (2.1,-4.1);
		\filldraw[fill=white,thick] (3.1,-3.1) circle (3pt);
		\node[text width=3cm] at (2.1,-0.3) {$a_1x  \geq b_1+1$};
		\node[text width=3cm] at (-0.7,-0.3) {$a_1x \leq b_1$};
		\node[text width=3cm] at (3.5,-1.7) {$a_2x \geq b_2 + 1$};
		\node[text width=3cm] at (5.4,-3.6) {$a_t x \geq b_t + 1$};
		\node[text width=3cm] at (2.2,-3.6) {$a_t x \leq b_t$};
		\node[text width=3cm] at (-0,-1.7) {$a_2x \leq b_2$};
		\node[text width=1cm] at (-0.7,-1.2) {$\emptyset$};
		\node[text width=1cm] at (0.4,-2.3) {$\emptyset$};
		\node[text width=1cm] at (4.65,-4.3) {$\emptyset$};
		\node[text width=1cm] at (2.4,-4.3) {$\emptyset$};
	\end{tikzpicture} 	
	\caption{A $\pSP$ refutation.}
\end{figure}


First, we establish the equivalence between $\CP$ and $\pSP$. 

\begin{lem}
	 $\pSP$ is polynomially equivalent to $\CP$. 	
\end{lem}
\begin{proof}
	Let $a_1x \geq b_1,\ldots, a_t x \geq b_t = 0\geq 1$ be the lines in a $\CP$ refutation of an unsatisfiable system of linear inequalities $F$ ordered such that $L_i \leq L_j$ if $L_i$ is derived using the line $L_j$. Let $P_0 = F$ and $P_i = P_{i-1} \cap \{a_ix \geq b_i\}$. 
	It can be verified that $P_i \cap \{a_ix \leq b_i-1\}= \emptyset$ and thus $P_0 \vdash \ldots \vdash P_t = \emptyset$ is a valid $\pSP$ refutation of $F$.
	
	Let $F=P_0, \ldots, P_t$ be a $\pSP$ refutation of $F$. Suppose that for all $i \in [t]$, $P_i$ is derived from $P_{i-1}$ by the $\pSP$ inference $a_ix \geq b_i$. By induction, suppose that there is $O(\ell)$-size $\CP$ derivation of $a_ix \geq b'_i$ for some $b'_i \geq b_i$ for every $i \leq \ell-1$ for some $\ell \in [t]$. Let $P'_{\ell-1} := F \cap_{i \leq \ell-1} \{a_ix \geq b'_i\}$ be the polytope formed by the inequalities derived so far. We will consider two cases based on whether $a_\ell x \geq b_\ell$ is valid for $P_{\ell-1}^*$. If $a_\ell x \geq b_\ell$ is valid for $P_{\ell-1}'$ then (by Farkas' Lemma) there exists $b_\ell' \geq b_\ell$ such that $a_\ell x \geq b_\ell'$ is a non-negative linear combination of the facets of $P_{\ell-1}'$ and thus can be derived by the linear combination rule. 
	
	If this is not the case then there must exist there exists $0<\varepsilon <1$ such that $a_\ell x \geq b_\ell-\varepsilon$ is valid for $P_{\ell-1}'$. This follows because $P_{\ell} \subset P_{\ell-1}' \subseteq P_{\ell-1}$ and $P_{\ell-1} \cap \{a_\ell x \leq b_\ell - 1\} = \emptyset$ because $a_\ell x \geq b_\ell$ is a $\pSP$ inference from $P_{\ell-1}$. Because $a_\ell x \geq b_\ell-\varepsilon$ is valid for $P_{\ell-1}'$, by Farkas' Lemma there exists $b_\ell' \geq b_\ell - \varepsilon$ such that $a_\ell x \geq b_\ell' $ is a non-negative linear combination of the facets of $P_{\ell-1}'$, and therefore $a_\ell x \geq \lceil b'_\ell\rceil$ can be derived by $\CP$. It follows that
	\[
	 	P_{\ell}' = P_{\ell-1}' \cap \{ a_\ell x \geq \lceil b'_\ell\rceil\} \subseteq P_{\ell-1} \cap \{a_\ell x \geq \lceil b_\ell - \varepsilon \rceil \}  \subseteq P_{\ell-1} \cap \{a_\ell x \geq b_\ell \} = P_\ell. \qedhere
	\]
\end{proof}


==> old-intro.tex <==
\newpage


The problem of refuting unsatisfiable systems of linear equations over a field $\mathbb{F}$ plays a central role in propositional proof complexity.
Indeed, such systems already appear in one of the first papers in the field: Tseitin's landmark 1968 paper \cite{tseitin68} that was arguably the first to study the optimal size of propositional proofs!
In his paper Tseitin introduced the following system of $\mathbb{F}_2$-linear equations, now called the \emph{Tseitin graph formulas}.
Let $G = (V, E)$ be a graph and let $\ell: V \rightarrow \mathbb{F}_2$ be a labelling of the vertices of $V$.
The Tseitin formula of $(G, \ell)$, denoted $\tsei(G, \ell)$, is the following system of $\mathbb{F}_2$-linear equations.
The system has a variable $x_e$ for each edge $e \in E$, and for each vertex $v$ we have the equation
\[ \bigoplus_{u: uv \in E} x_{uv} = \ell(v)\]
asserting that the sum of the edge variables
incident with $v$ must agree with its label $\ell(v)$.
It is easy to see by the handshaking principle that for any connected $G$ the system of equations $\tsei(G, \ell)$ is unsatisfiable if and only if the sum of all labels is odd.
Tseitin used these formulas on grid graphs to prove the first strong lower bounds on the length of \emph{regular} Resolution refutations \cite{tseitin68}.

Since Tseitin's early work, his formulas have been tightly woven with many major results in propositional proof complexity.
In particular, they have played an important role in the development of lower bound techniques through the use of \emph{expansion}, which is now one of the major tools in the field. 
%central role of expansion appears in many early papers mention Galil established regular resolution lower bounds on Tseitin formulas on expander graphs , Urquhart Tseitin for regular, Avi, Chvatal. Establishing lower bounds for Tseitin as well as random expanding CNF instances.
The use of expansion in this way was pioneered in \cite{galil1, urq87, BenSassonW01}. Urquhart~\cite{urq87}, building on \cite{galil1}, established that Tseitin formulas on expander graphs are hard for Resolution. This was generalized by Ben-Sasson and Wigderson~\cite{BenSassonW01} who showed that almost all known Resolution lower bounds follow from expansion. 
%that expansion could be used more broadly as a unifying hardness parameter for Resolution.
%The use of expansion in this way was pioneered by Urquhart \cite{urq87}, who established that Tseitin formulas on expander graphs are hard for general Resolution.
Subsequently, lower bounds on Tseitin formulas for expanders were established for many other major propositional proof systems, including Nullstellensatz \cite{dima-nsatz},
Polynomial Calculus \cite{bgip}, Sum-of-Squares \cite{dima-sos,Schoenebeck08}, and bounded-depth Frege \cite{Ben-Sasson02,PitassiRST16,hastad-grid,GalesiIRS19}.

Due to this relationship with graph expansion, it should come as no surprise that the proof complexity of Tseitin instances is closely related to the proof complexity of \emph{random CNF formulas}.
Given positive integers $m, n, k$ let $\mathcal{F}(m, n, k)$ denote the distribution over $k$-CNF formulas obtained by choosing $m$ clauses of width $k$ over a set of $n$ variables, each sampled uniformly at random with replacement.
It is known that if the \emph{clause density} $\Delta = m/n$ is greater than roughly $2^k \ln 2$ then a sample $F \sim \mathcal{F}(m, n, k)$ will be unsatisfiable with high probability; it is widely conjectured in proof complexity that random formulas with density near this $2^k \ln 2$ threshold are hard to refute by \emph{any} propositional proof system.
This conjecture has been verified for many propositional proof systems of interest; furthermore, such verification has almost always been preceded by proving lower bounds on Tseitin formulas first.
Indeed, Urquhart's lower bound for Tseitin instances led to
Chv\'atal and Szemeredi's exponential lower bounds for general Resolution refutations of random $k$-CNF formulas \cite{cs-resolution}, and similarly for many other proof systems including Nullstellensatz, Polynomial Calculus, SOS, and bounded-depth Frege \cite{Ben-Sasson02,dima-nsatz,dima-sos,PitassiRST16,hastad-grid}.

%By varying the underlying odd-labelling and $k$-regular graph, we get precisely
%a uniform distribution on $k$-XOR instances where each variable occurs exactly twice.
%Because of this connection, lower bounds for Tseitin instances have been a precursor
%to lower bounds for random instances, such as random $k$-XOR and random $k$-SAT.
\paragraph{Cutting Planes Proofs and Tseitin Formulas.} 
There is, however, one prominent exception to the above discussion: the \emph{Cutting Planes} proof system.
Cutting Planes proofs reason about integral solutions to linear systems of equations.
Formally, given a system of integer-linear inequalities $Ax \geq b$ a \emph{Cutting Planes proof} of an inequality from the system is given by a sequence of inequalities $P = \set{a_i x \geq c_i}_{i \in [s]}$ such that every inequality $a_i x \geq c_i$ is either in $Ax \geq b$ or is deduced from earlier inequalities in the sequence by one of the following two deduction rules:
\begin{itemize}
	\item {\emph{Conic Combination.}} From any set of inequalities $f_1, \ldots, f_k$ deduce $\sum_{i=1}^k \lambda_i f_i$, where $\lambda_i$ are non-negative integer coefficients.
	\item {\emph{Rounding.}} From the inequality $ax \geq b$ and any integer $d$ dividing each entry of $a$, deduce $(a/d)x \geq \lceil b/d \rceil$.
\end{itemize}
Note that while the first rule is sound over any solutions to the system, the second rule is only sound over integer solutions.
A \emph{Cutting Planes refutation} of $Ax \geq b$ is a proof of the inequality $0 \geq 1$ from $Ax \geq b$; such a proof exists if and only if $Ax \geq b$ has no integer-valued solutions.

The Cutting Planes proof system was originally introduced and studied in the context of integer-linear programming by Gomory~\cite{gomory1963algorithm} and Chvat\'{a}l \cite{Chvatal73a}, and then formalized as a propositional proof system by Cook, Cuillard, and Tur\'an \cite{CookCT87}, who also conjectured that Tseitin formulas should be hard for Cutting Planes.
%generalized \cite{krajicek,stabbing planes}.
Exponential lower bounds for Cutting Planes were established in the 90s
for the clique-colouring formulas\cite{Pudlak97,HakenC99} (see also \cite{Krajicek97,razborov1995unprovability,BonetPR97}) and, much more recently, for random $O(\log n)$-width random CNF formulas \cite{FlemingPPR17,HrubesP17}.
This state of affairs is out of order with the usual progression of proof complexity, in which Tseitin lower bounds are proven first (usually by exploiting expansion), and these techniques enable studying random CNF formulas.
It suggests a basic and intriguing question: can formal reasoning about linear inequalities over the \emph{reals} efficiently simulate reasoning about linear equalities over \emph{finite fields}?

In a recent breakthrough, Dadush and Tiwari  \cite{TseitinUpperBound} gave \emph{quasipolynomial-size} Cutting Planes refutations of Tseitin instances, thereby \emph{refuting} the longstanding conjecture that they require exponential size.  
In light of the known exponential lower bounds for random CNF formulas, Dadush and Tiwari's result highlights an interesting contrast between Cutting Planes and the other proof systems discussed above.
In particular, there is an \emph{exponential gap} in the ability of Cutting Planes to refute systems of $\mathbb{F}_2$-linear equations versus random CNF formulas. 
This shows that Cutting Planes can reason about equations over finite fields much more efficiently than was previously conjectured.

%Moreover, lower bounds for Tseitin formulas
%has gone hand-in-hand with proving similar bounds for
%any expanding family of formulas, including random mod-2 equations
%and random kCNF equations.

\paragraph{Our results.}   In this work, we complement the result of Dadush and Tiwari with new upper and lower bounds, which taken together give a more complete picture of the ability of Cutting Planes procedures to reason about systems of linear equations:

\begin{enumerate}
	\item First, we prove optimal depth (also known as rank) lower bounds for a strong generalization of Cutting Planes known as \emph{semantic Cutting Planes}, which includes Cutting Planes %and Lovasz-Schrijver (LS) 
	as a special case.  
		Indeed, we show that linear depth lower bounds hold for semantic Cutting Planes refutations of Tseitin, random $\mathbb{F}_2$-linear equations, and random $k$-CNF instances.   
		Our new depth bounds can also be used to prove integrality gaps, as well as a new method to lift lower bounds on Resolution depth to lower bounds on semantic Cutting Planes depth, which may be of independent interest.

	\item In contrast, we show that that the Stabbing Planes proof system introduced by Beame et. al.~\cite{BeameFIKPPR18}, which is a natural generalization of Cutting Planes, admits \emph{quasi-polynomial} size and $O(\log^2 n)$-depth refutations of \emph{any} unsatisfiable system of linear equations over a finite field.

	\item Finally, via a new equivalence we prove between Cutting Planes and a fragment of Stabbing Planes, we show how to ``recompile'' any Stabbing Planes proof with a particular structure into a Cutting Planes proof of the same size (but, crucially, not of the same depth).
		This simulation allows us to transform our Stabbing Planes upper bounds into quasipolynomial-size Cutting Planes refutations for any unsatisfiable system of linear equations, which gives an alternate exposition of the result of Dadush and Tiwari~\cite{TseitinUpperBound}. 
		Our simulation also allows us to show that \emph{any} Stabbing Planes proof with bounded coefficients can be quasi-polynomially simulated by Cutting Planes.
		Together with the known lower bounds for Cutting Planes~\cite{Pudlak97,FlemingPPR17,HrubesP17}, this establishes the first exponential lower bounds on Stabbing Planes refutations with bounded coefficients of CNF formulas. 
\end{enumerate}
Prior to our work,~\cite{BGHMP06} established linear rank lower bounds for the instances that we study, but no rank bounds for general semantic Cutting Planes refutations of these instances were known.  
Our second result extends the work of Beame et al.~\cite{BeameFIKPPR18}, who showed that Stabbing Planes admits quasipolynomial-size proofs of Tseitin instances.



\begin{conj}
	There is a family of Tseitin instances $(G_n, \ell_n)$ such that any Cutting Planes refutation of $\tsei(G_n, \ell_n)$ in \emph{subexponential} size $2^{n^{o(1)}}$ requires \emph{superlinear} depth $\omega(n)$.
\end{conj}

We also note that these proofs are DAG-like, and it is open whether or not these proofs can be made tree-like.
We conjecture that this is \emph{not} true:

\begin{conj}
	There is a family of Tseitin instances $(G_n, \ell_n)$ such that any \emph{tree-like} Cutting Planes refutation of $\tsei(G_n, \ell_n)$ requires exponential size.
\end{conj}

%
% showing
%that a broad
%class of threshold logic proof systems called {\it semantic} Cutting Planes
%(which includes Cutting Planes and the Lovasz-Schrijver (LS) systems
%as special cases) cannot have both small and shallow refutations
%for $\bmod 2$ equations.
%On the other hand, we show that a natural generalization of Cutting Planes,
%Stabbing Planes, does admit short and shallow refutations.
%
%\begin{enumerate}
%\item First, we prove linear rank lower bounds for
%any {\it semantic} Cutting Planes refutation of Tseitin, random $\bmod 2$ and random $k$-CNF
%instances. Our proof method is a new topological argument that we instantiate
%to prove rank bounds and integrality gaps for random instances, as well
%as for any family of lifted tautologies satisfying certain properties.
%\item In contrast, we present low-depth and small-size refutations
%in the Stabbing Planes proof system, which is a natural generalization of
%Cutting Planes.
%\item Adapting the breakthrough upper bound of Dadush and Tiwari 
%\cite{TseitinUpperBound},
%we also give quasipolynomial-size Cutting Planes refutations for any unsatisfiable system of $\bmod p$ equations.
%\end{enumerate}
%
%Prior to our work, linear rank lower bounds for Tseitin and
%random formulas were known
%for the case of Cutting Planes refutations \cite{BGHMP06}, 
%not for general semantic Cutting Planes refutations.
%
%These results taken together give a more complete picture of
%the ability of Cutting Planes procedures to refute linear equations.
%It is interesting to note that in contrast to the
%other proof systems discussed above, Cutting Planes displays an
%exponential gap in its ability to refute random $\bmod 2$ formulas
%versus random CNF formulas.
%Random $\bmod 2$ formulas can be refuted in quasi-polynomial time,
%whereas the latter were recently shown to require exponential size Cutting Planes proofs \cite{FlemingPPR17,HrubesP17}.

\subsection{Related Work}
Lower bounds on subsystems of $\SP$ and its dag-like variant $\RCP$ have been established in earlier works. Kraj\'{i}\u{c}ek \cite{Krajicek98} proved exponential lower bounds on $\RCP$ proofs in which both the \emph{width} of the clauses and the magnitude of the coefficients of each line in the proof are bounded. Concretely, let these bounds be $w$ and $c$ respectively. The lower bound that he obtains is $2^{n^{\Omega(1)}}/c^{w \log^2 n}$. Kojevnikov \cite{Kojevnikov07} removed the dependence on the coefficient size for $\tRCP$ proofs, obtaining a bound of $\exp(\Omega(\sqrt{n/w \log n}))$. A depth $d$ $\SP$ refutation implies a width $d$ $\tRCP$ refutation of  the same size \cite{BeameFIKPPR18}, %there are width-1 tRCP refutations of every formula (as CP is complete) however there are no depth n/log n refutations of certain formulas in SP} 
and therefore this implies lower bounds on the size of $\SP$ proofs of depth $o(n/\log n)$. Beame et al. \cite{BeameFIKPPR18} exhibit a function for which there \emph{do not exist} $\SP$ refutations of depth $o(n / \log^2 n)$ via a reduction to the communication complexity of the CNF search problem. %; this can be improved to,






==> oldConversionToLinSP.tex <==

	%We now show that certain ``structured'' $\SP$ proofs --- like the one in Section~\ref{sec:qpSPref} --- can be converted into $\CP$ proofs of comparable size. 


\begin{defn}
	A Stabbing Planes query $(ax \leq b-1, ax \geq b)$ at a node corresponding to a polytope $P$ is \emph{pathlike} if at least one of $P \cap \{x: ax \leq b-1\}$ and $P \cap \{x: ax \geq b\}$ is empty (see \autoref{fig:pSPqueries}). A Pathlike $\SP$ refutation is one in which every query is pathlike. 
\end{defn}

The name ``pathlike'' stems from the fact that the underlying graph of a pathlike Stabbing Planes proof is a path, since at most one child of every node has any children. 
Equivalently, at least one of $ax \leq b$ or $ax \geq b-1$ must be \emph{valid} for the polytope $P$, meaning that every (real) $x \in P$ satisfies the inequality. 
In contrast, facelike queries relax that requirement, and only enforce that one child is either empty or a face of $P$.

\begin{figure}[htbp]
	\centering
	\begin{subfigure}[b]{1\textwidth}
	\begin{tikzpicture}[scale=0.6]
		\draw[thick, ->] (-2,5)  -- (-0.5,3.5);
		\draw[thick, ->] (-2,5)  -- (-3.5,3.5);
		\filldraw[fill=green!9,thick] (-2,5) circle (8pt);
		\node[text width=2cm] at (0.5,4.4) { $ax \geq b$};
		\node[text width=2cm] at (-4.3,4.4) {$ax \leq b-1$};
		%little arrows
		%\draw[thick, dashed, ->] (1.65,2.83)  -- (2.05,2.39);
		\filldraw[fill=red!15,thick] (-3.75,3.2) circle (10pt);
		\node[text width=1cm] at (-3.14,3.2) { $\emptyset$};
		\draw[thick, ->,dashed] (-0.4,3.35)  -- (1.1,1.85);
		\draw[thick, ->] (-0.4,3.35)  -- (-1.9,1.85);
		%\node[text width=2cm] at (-6.2,2.7) {$a_2x \leq b_2-1$};
		%\node[text width=2cm] at (-1.1,2.7) {$a_2x \geq b_2$};
		\filldraw[fill=green!9,thick] (-0.35,3.25) circle (8pt);
		\filldraw[fill=red!15,thick] (-2.05,1.5) circle (10pt);
		\node[text width=1cm] at (-1.4,1.5) { $\emptyset$};
		%\draw[thick, dashed]  (-5.15,1.85) -- (-6.65,0.35);
		%\draw[thick, ->] (-6.65,0.35)  -- (-8.15,-1.15);
		%\draw[thick, ->] (-6.65,0.35)  -- (-5.15,-1.15);
		%\filldraw[fill=green!9,thick] (-6.65,0.35) circle (7pt);
		
		%\filldraw[fill=red!15,thick] (-2,1.5) circle (9pt);
		%\node[text width=1cm] at (-1.35,1.5) { $\emptyset$};
		
		%\filldraw[fill=red!15,thick] (-5,-1.4) circle (9pt);
		%\node[text width=1cm] at (-4.35,-1.4) { $\emptyset$};
		
		%\filldraw[fill=red!15,thick] (-8.3,-1.4) circle (9pt);
		%\node[text width=1cm] at (-7.65,-1.4) { $\emptyset$};
		
		%\node[text width=2cm] at (-9.1,-0.3) {$a_sx \leq b_s-1$};
		%\node[text width=2cm] at (-4.1,-0.3) {$a_sx \geq b_s$};	
		\node[text width=2cm] at (-4.6,0) {\phantom{a}};	
	\end{tikzpicture} \hspace{1.3em}
	\begin{tikzpicture}[scale=0.6]
	\filldraw[color=black!60, fill=green!9, very thick] (6.4,-0.5)-- (3.8,0.7) -- (3.9,3.2) -- (6.3,4.5) -- (8.8,3.2) -- (8.7,0.5) -- cycle;
	\filldraw[color=white, fill=white!, very thick,opacity=0.7] (3.1,5.3)  -- (3.86,-1.5)  -- (4.6,-1.4) -- (4.55,5.4) -- cycle;
	%\draw[color=red!50, very thick] (3.6,0.7) -- (3.7,3.2);
	%\draw[color=betterYellow!80, very thick] (3.6,0.7) -- (6.2,-0.5);
	\draw[color=black!60, very thick] (3.4,5.3)  -- (3.4,-1.5);
	\draw[color=black!60, very thick,->] (4.6,2)  -- (4.9,2);
	\draw[color=black!60, very thick] (4.6,5.4)  -- (4.6,-1.4);
	\draw[color=black!60, very thick,->] (3.4,2)  -- (3.1,2);
	\node[text width=3cm] at (2.5,2) {$ax \leq b-1$};
	\node[text width=3cm] at (7.7,2) {$ax \geq b$};
	\node[text width=1cm] at (6.7,4) {$P$};
	\end{tikzpicture}
	\caption{A Pathlike query. The polytope $P \cap \{x:ax \leq b-1\} = \emptyset$. }\label{fig:pSPqueries}
	\end{subfigure}
	
	
	\begin{subfigure}[b]{1\textwidth}
	\begin{tikzpicture}[scale=0.6]
		\draw[thick, ->] (-1,5)  -- (1.5,3.5);
		\draw[thick, ->] (-1,5)  -- (-3.5,3.5);
		\filldraw[fill=white,thick] (-1,5) circle (8pt);
		\node[text width=2cm] at (2,4.5) { $ax \geq b$};
		\node[text width=2cm] at (-3.6,4.5) {$ax \leq b-1$};
		%little arrows
		%\draw[thick, dashed, ->] (1.65,2.83)  -- (2.05,2.39);
		\draw[thick, ->, dashed] (1.65,3.35)  -- (2.65,2.35);
		\draw[thick, ->,dashed] (1.65,3.35)  -- (0.65,2.35);
		\filldraw[fill=green!9] (1.65,3.2) circle (8pt);
		\draw[thick, ->, dashed] (-3.65,3.35)  -- (-2.65,2.35);
		\draw[thick, ->,dashed] (-3.65,3.35)  -- (-4.65,2.35);
		\filldraw[fill=orange!30,thick,thick] (-3.65,3.25) circle (8pt);
		
		
		\node[text width=2cm] at (-4.6,0) {\phantom{a}};	
	\end{tikzpicture}
	\begin{tikzpicture}[scale=0.6]
	\filldraw[color=black!60, fill=green!9, very thick] (6.4,-0.5)-- (3.8,0.7) -- (3.9,3.2) -- (6.3,4.5) -- (8.8,3.2) -- (8.7,0.5) -- cycle;
	\filldraw[color=white, fill=white!, very thick,opacity=0.7] (3.1,5.3)  -- (3.86,-1.5)  -- (4.7,-1.4) -- (4.9,5.4) -- cycle;
	%\draw[color=red!50, very thick] (3.6,0.7) -- (3.7,3.2);
	%\draw[color=betterYellow!80, very thick] (3.6,0.7) -- (6.2,-0.5);
	\draw[color=black!60, very thick] (3.95,5.3)  -- (3.7,-1.5);
	\draw[color=black!60, very thick,->] (4.8,2)  -- (5.15,1.98);
	\draw[color=black!60, very thick] (4.95,5.4)  -- (4.7,-1.4);
	\draw[color=black!60, very thick,->] (3.8,2.01)  -- (3.48,2.029);
	\draw[color=orange!70, very thick] (3.78,0.7) -- (3.88,3.2);
	\node[text width=3cm] at (3,2) {$ax \leq b-1$};
	\node[text width=3cm] at (7.8,2) {$ax \geq b$};
	\node[text width=1cm] at (6.7,4) {$P$};
	\node[text width=3cm] at (3.8,-1.8) {$ax =b-1$};
	\end{tikzpicture}
	\caption{A Facelike query. The polytope $P \cap \{x:ax\leq b-1\} = P \cap \{x:ax=b\}$ is a face of $P$.} \label{fig:fSPqueries}
	\end{subfigure}
	\caption{Pathlike and Facelike $\SP$ queries on a polytope $P$. On the left are the proofs and on the right are the corresponding effects on the polytope.}
\end{figure} 

	Let $(ax \leq b-1, ax \geq b)$ be the query at a node corresponding to a polytope $P$ in a Pathlike $\SP$ proof, and suppose that $P \cap \{x: ax \leq b-1\} = \emptyset$. 
	In this case, we will say that $ax \geq b$ is a Pathlike $\SP$ \emph{inference} from $P$, and denote the inference by $P \vdash P \cap \{x: ax \geq b\}$. 
	Thus, we can view a Pathlike $\SP$ refutation of an unsatisfiable system of linear inequalities $Ax \geq b$ as a sequence of polytopes $\{x: Ax \geq b\} = P_0, \ldots, P_s = \emptyset$ such that $P_i \vdash P_{i+1}$. 
	For simplicity of notation, throughout this section we will denote $\{x: ax \geq b\}$ by $\{ax \geq b\}$.
	
\begin{lem}
	 Pathlike $\SP$ is polynomially equivalent to $\CP$. 	
\end{lem}
\begin{proof}
	First we show how to simulate a $\CP$ refutation in a Pathlike $\SP$. 
	Let \[a_1x \geq b_1, a_2x \geq b_2, \ldots, a_sx \geq b_s\] be a $\CP$ refutation of an unsatisfiable system of linear inequalities $Ax \geq b$. 
	Consider the sequence of polytopes $P_0 =\{Ax \geq b\}$ and $P_i = P_{i-1} \cap \{a_i x \geq b_i\}$. 
	By inspecting the rules of $\CP$, it can observed that $P_i \cap \{a_ix \leq b_i-1\}= \emptyset$ and thus $P_i \vdash P_{i+1}$ for all $0 \leq i \leq s$.
	
	Next, let $\{Ax \geq b\} = P_0,\ldots, P_s = \emptyset$ be a Pathlike $\SP$ refutation of any unsatisfiable system of linear inequalities $Ax \geq b$. For all $i \in [s]$ let $P_i$ be deduced from $P_{i-1}$ by the Pathlike $\SP$ inference $a_ix \geq b_i$. Let $t \in [s-1]$ and suppose by induction that there is a $\CP$ derivation $D$ of size at most $2t$ of an inequality $a_t x \geq b_t'$ for some $b_t' \geq b_t$, and further that for every $i \in [t]$, the derivation $D$ contains an inequality $a_i x \geq b_i'$ for $b_i' \geq b_i$. That is, the polytope $P_D$ formed by the intersection of the halfspaces of $D$ is contained within $P_t$. We show how to derive an inequality $a_{t+1} x \geq b_{t+1}'$ for $b_{t+1} \geq b_{t+1}$.
	
	We consider two cases. First, if $a_{t+1} x \geq b_{t+1}$ is valid for $P_D$ then by Farkas' Lemma, there exists $b_{t+1}' \geq b_{t+1}$ such that $ax \geq b_{t+1}'$ can be written as a conic combination of the inequalities in $D$, and so it can be derived by a single application of the conic combination rule.
	 
	Otherwise, we must use the division rule as well. In this case $P_D \cap \{ax < b_{t+1}\} \neq \emptyset$ and because $P_D \subseteq P_t$ and $P_t \cap \{ax \leq b-1\} = \emptyset$. From this it  follows that there exists $0 < \varepsilon < 1$ such that $a_t x\geq b_t - \varepsilon$ is valid for $P_D$. It follows by Farkas' Lemma that there exists $b_{t+1}' \geq b_{t+1} - \varepsilon$ such that $ax \geq b_{t+1}'$ can be written as a conic combination of the inequalities in $D$. Therefore $ax \geq \lceil b_{t+1} \rceil$ can derived division from $D$ in $\CP$. Observe that 
	\[ \lceil b_{t+1}'  \rceil \geq \lceil b_{t+1} -\varepsilon \rceil =b_{t+1}, \]
	because $b_{t+1} \in \mathbb{Z}$ and $\varepsilon < 1$. 
	It follows that
	\[ P_D \cap \{ a_{t+1} x \geq \lceil b_{t+1}'\rceil \} \subseteq P_t \cap \{ a_{t+1} x \geq \lceil b_{t+1}'\rceil \} \subseteq P_t \cap \{a_{t+1} x \geq b_{t+1}\} = P_{t+1}. \qedhere \]
\end{proof}
		
	Next, we show how to simulate Facelike $\SP$ proofs by Pathlike $\SP$ proofs of comparable size.
	The proof of \autoref{lem:SPtopSP} is inspired by the work of Dadush and Tiwari \cite{TseitinUpperBound}, and will use the following lemma due to Shrijver~\cite{SCHRIJVER1980291} (a proof can be found in \CITE{CCT87}).
	\begin{lem}
	\label{lem:fSPtopSP}
		Let $P$ be a polytope defined by an integral system and let $F$ be a facet of $P$. If $F \vdash F'$ then there is a polytope $P'$ such that $P \vdash P'$ and $P' \cap F \subseteq F'$.
	\end{lem}
%	\begin{proof}
		%Let $P = \{Ax \leq b\}$ and $F = \{A_0x = b_0, A_1x \leq b_1\}$. Suppose $F' = F \cap \{ax \leq b\}$ is obtained by the Pathlike $\SP$ inference $ax \leq b$. Since $F \cap \{ ax \geq b+1\}$ is empty, there is some $0 <\varepsilon < 1$ such that $ax \leq b+ \varepsilon$ is valid for $F$. It follows that there are vectors $y_0,y_1$ such that $y_1 \geq 0$ and 
		%\begin{align*}
		%	y_0A_0 + y_1A_1 &=a \\
		%	y_0 b_0 + y_1 b_1&\leq b + \varepsilon.
		%\end{align*}
		%Let $z_0$ be any integral vector such that $y_0 - z_0$ is non-negative --- for instance, we could choose $z_0 = \lfloor y_0 \rfloor$. 
		%%Let $a' = a - z_0 A_0$ and $b' = b- z_0b_0$. 
		%Observe that $a'x \leq b' + \varepsilon$ is valid for $P$ as it can be deduced from $P$ since $y_0-z_0$ is non-negative. 
		%Indeed, we have shifted $ax \leq b + \varepsilon$ so that it no longer depends on the inequalities in $A_0x \geq b_0$. Let $P' := P \cap \{ a'x \leq b'  \}$, noting that $P \vdash P'$ as $a'$ and $b'$ are integral and $P \cap \{a'x \geq b' + 1\}  = \emptyset$ because $a'x \leq b'+\varepsilon$ is valid for $P$. 
	%	
	%	Let $x \in P' \cap F$, and thus $x \in F$ and $a'x \leq b'$. Expanding $a'$ and $b'$ we have 
	%	\[a'x = (a-z_0A_0)x \leq b' = b - z_0b_0. \]
	%	Rearranging we have that $a'x \leq b'$ implies that 
	%	\[ ax \leq b + z_0(A_0x-b_0). \]
	%	However since $x \in F$, $A_0x = b_0$ and thus $ax \leq b$, implying that $x \in F'$. 
	%\end{proof}
	
	\begin{lem}
	\label{lem:SPtopSP}
		Facelike $\SP$ is polynomially equivalent to Pathlike $\SP$.	
	\end{lem}
	Let $\pi$ be a Facelike $\SP$ refutation of size $s$ refuting a CNF formula $F$. 
	Then there is a size $s$ $\CP$ refutation of $F$. 
	For a polytope $P$, a hyperplane $ax = b$ is \emph{supporting} if $b = \max \{ ax : x \in P\}$. If $ax = b$ is a supporting hyperplane then $P \cap \{ax = b\}$ is called a \emph{face} of $P$, and is itself a polytope (albeit of lower dimension). Equivalently, if $P=\{x: Ax \leq b\}$, then a set $F$ is a face if and only if there is a partition of the constraints into $A_0x \leq b_0$ and $A_1x \leq b_1$ such that $F =\{x \in P: A_0x = b_0, A_1x \leq b_1\}$ . This follows readily from linear programming duality.
	
	We are now ready to prove \autoref{lem:SPtopSP}. We say that a polytope $P'$ has a Pathlike $\SP$ \emph{derivation} in $t$ queries from a polytope $P$ if there exists a sequence of polytopes $P=P_0,\ldots, P_{t+1} \subseteq P'$ such that $P_i \vdash P_{i+1}$ for $i \in [t]$.
	The key is the following claim, which will enable our recursive case. 
	
	\spcnoindent
	{\bf Claim.} Let $P$ be a polytope and $ax \geq b$ be valid for $P$. Assume that $P \cap \{ax = b\}$ has a Pathlike $\SP$ refutation with $t$ queries. Then there is a Pathlike $\SP$ derivation of $P \cap \{ax \geq b\}$ in $t+1$ queries from $P$. 
	\begin{proof}[Proof of Claim.]
		Since $ax \geq b$ is valid for $P$, it follows that $F = P \cap \{ax = b\}$ is a face of $P$. Consider the Pathlike $\SP$ refutation $F = F_0 \vdash F_1 \vdash \cdots \vdash F_t = \emptyset$. Applying the above lemma repeatedly, we get a sequence of polytopes $P = P_0 \vdash P_1 \vdash \cdots \vdash P_t$ such that $P_i \cap F = P_i \cap \{ax = b\} \subseteq F_i$. Thus $P_t \cap \{ax = b\} \subseteq F_t = \emptyset$ and $ax \geq b+1$ is Pathlike $\SP$ inference for $P_t$. This means that $P_t \vdash P_t \cap \{ax \geq b+1\} \subseteq P \cap \{ax \geq b+1\}$.
	\end{proof}
	
	That Facelike $\SP$ simulates Pathlike $\SP$ follows by the fact that any Pathlike $\SP$ query is a valid query in Facelike $\SP$.  
	For the other direction, consider a $\SP$ refutation $\pi$ of size $t$. 
	We generate a Pathlike $\SP$ refutation by the following recursive algorithm, which performs an \emph{in-order} traversal of $\pi$. 
	At each step of the recursion (corresponding to a node in $\pi$) we maintain the current polytope $P$ we are visiting and a Pathlike $\SP$ proof $\Pi$ --- initially, $P$ is the polytope corresponding to the input CNF formula and $\Pi = \emptyset$. 
	We maintain the invariant that when we finish the recursive step at node $P$, the Pathlike $\SP$ refutation $\Pi$ is a refutation of $P$. 
	
	We are now ready to describe the algorithm. Initially, set $P$ to be the polytope from our input CNF formula and $P$. Then
	\begin{enumerate}
		\item Let $(ax \leq b,~ ax \geq b+1)$ be the current query and suppose that $ax \geq b$ is valid for $P$.
		\item Recursively refute $P \cap \{ ax \leq b\}$, obtaining a Pathlike $\SP$ refutation $\Pi$ with $t$ queries. 
		\item Apply the Claim to deduce $P \cap \{ax \geq b+1\}$ from $P$ in $t+1$ queries. 
		\item Refute $P \cap \{ ax \geq b+1\}$ by using the $\SP$ refutation for the right child. 
	\end{enumerate}
	Correctness follows immediately from the Claim, as well as the size of the resulting proof is the same as the size of the $\SP$ refutation. 		
	\end{proof}
	
	\autoref{thm:main} follows by combining \autoref{lem:SPtopSP} with \autoref{lem:fSPtopSP}.

